Tracking Employment Shocks Using Mobile Phone Data

Can data from mobile phones be used to observe economic shocks and their consequences at multiple scales? Here we present novel methods to detect mass layoffs, identify individuals affected by them, and predict changes in aggregate unemployment rates using call detail records (CDRs) from mobile phones. Using the closure of a large manufacturing plant as a case study, we first describe a structural break model to correctly detect the date of a mass layoff and estimate its size. We then use a Bayesian classification model to identify affected individuals by observing changes in calling behavior following the plant's closure. For these affected individuals, we observe significant declines in social behavior and mobility following job loss. Using the features identified at the micro level, we show that the same changes in these calling behaviors, aggregated at the regional level, can improve forecasts of macro unemployment rates. These methods and results highlight promise of new data resources to measure micro economic behavior and improve estimates of critical economic indicators.

==> RMSE_fe.tex <==
\begin{table*}[htbp]\centering
{\fontsize{7pt}{7pt}\selectfont
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{RMSE with the addition of CDR data from the entire quarter with various fixed effects. The best performing model is bolded.}
\label{tab:rmse_fe_full}
\begin{tabular}{l*{10}{c}}
\hline \hline \\
	& \multicolumn{3}{c}{No F.E.} & \multicolumn{3}{c}{Quarter F.E.} & \multicolumn{3}{c}{Province F.E.} \\
Model & RMSE & RMSE w/ CDR & $\Delta$RMSE\% & RMSE & RMSE w/ CDR & $\Delta$RMSE\% & RMSE & RMSE w/ CDR & $\Delta$RMSE\% \\
\hline
Present & & & & & & & & \\
AR1	& 0.0192 & 0.0168 & 12.37 & 0.195 & 0.0179 &  8.18 & 0.0217 & 0.0171 & 21.34 \\
AR1 Quad	& 0.0191 & 0.0168 & 11.88 &  0.0190 &  0.0178 &  6.23 & 0.0218 & 0.0171 &  21.18 \\
AR1 GDP	& 0.0173 & \textbf{0.0166} &  3.93 & 0.0178 & 0.0176 & 0.89 & 0.0179 & 0.0168 & 6.24 \\
\hline
Future & & & & & & & & \\
AR1	& 0.0315 & 0.0257 & 18.45 & 0.0315 & 0.0281 & 10.76 & 0.0365 & 0.0318 & 12.92 \\
AR1 Quad & 0.0308 & 0.0262 & 14.89 & 0.0302 & 0.0285 &  5.55 & 0.0358 & 0.0314 & 12.21 \\
AR1 GDP & 0.0260 &  \textbf{0.0246} & 5.37  &  0.0270 &   0.0269 &   0.61 & 0.0274 & 0.0313 &  -14.12 \\
\\
\hline \hline
\end{tabular}}
\end{table*}

\begin{table*}[htbp]\centering
{\fontsize{7pt}{7pt}\selectfont
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{RMSE with the addition of CDR data from the half of the quarter with various fixed effects. The best performing model is bolded.}
\label{tab:rmse_fe_half}
\begin{tabular}{l*{10}{c}}
\hline \hline \\
	& \multicolumn{3}{c}{No F.E.} & \multicolumn{3}{c}{Quarter F.E.} & \multicolumn{3}{c}{Province F.E.} \\
Model & RMSE & RMSE w/ CDR & $\Delta$RMSE\% & RMSE & RMSE w/ CDR & $\Delta$RMSE\% & RMSE & RMSE w/ CDR & $\Delta$RMSE\% \\
\hline
Present & & & & & & & & \\
AR1	& 0.0192 & 0.0164 & 14.04 & 0.0194  & 0.0172 &  11.12 & 0.0217  & 0.0165  & 23.82 \\
AR1 Quad	&  0.0190  & \textbf{0.0163} & 14.19 & 0.0189   & 0.0170 & 10.01 & 0.0217  & 0.0164  & 24.58 \\
AR1 GDP	& 0.0173  & 0.0165  & 4.49 & 0.0177  & 0.0175  & 1.08 & 0.0179  & 0.0165 & 7.51 \\
\hline
Future & & & & & & & &  \\
AR1	&  0.0314 & 0.0258 &  17.80 & 0.0315 & 0.0273  & 13.07 & 0.0365  & 0.0267 &  26.73936 \\
AR1 Quad & 0.0307  & \textbf{0.0246}  & 19.77 & 0.0301  & 0.0262  & 13.02 & 0.0357  & 0.0256  & 28.36 \\
AR1 GDP & 0.0259  & 0.0258  & 0.50 & 0.0270  & 0.0270  &  -0.046& 0.0274  & 0.0272  & 0.49\\
\\
\hline \hline
\end{tabular}}
\end{table*}


==> call_var_correlation.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Correlation coefficients between normalized, aggregated calling behaviors and unemployment rates the province level. Pairwise correlations between metrics are done quarterly for each province giving a total of 416 observations for each variable comparison}
\label{tab:PCA_corr}
\begin{tabular}{l*{8}{c}}
\hline\hline
                &\multicolumn{8}{c}{(1)}                                                                                                                                \\
                &\multicolumn{8}{c}{}                                                                                                                                   \\
                &Calls         &Inc         &Out         &Contacts         &Churn         &Towers         &$R_g$         &Unemp         \\
\hline
Calls       &        1         &                  &                  &                  &                  &                  &                  &                  \\
Inc       &    0.746\sym{***}&        1         &                  &                  &                  &                  &                  &                  \\
Out       &    0.952\sym{***}&    0.724\sym{***}&        1         &                  &                  &                  &                  &                  \\
Contacts       &    0.807\sym{***}&    0.667\sym{***}&    0.858\sym{***}&        1         &                  &                  &                  &                  \\
Churn       &    0.102\sym{*}  &   -0.141\sym{**} &    0.132\sym{**} &    0.183\sym{***}&        1         &                  &                  &                  \\
Towers       &    0.701\sym{***}&    0.522\sym{***}&    0.711\sym{***}&    0.584\sym{***}&    0.196\sym{***}&        1         &                  &                  \\
$R_g$       &    0.373\sym{***}&    0.193\sym{***}&    0.379\sym{***}&    0.269\sym{***}&    0.177\sym{***}&    0.696\sym{***}&        1         &                  \\
Unemp       &   -0.428\sym{***}&   -0.356\sym{***}&   -0.396\sym{***}&   -0.169\sym{***}&    0.138\sym{**} &   -0.418\sym{***}&   -0.295\sym{***}&        1         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table*}


==> duhat_prediction.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption*{Predicting in-sample changes in quarterly unemployment rates}
\begin{tabular}{l*{1}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}\\
            &\multicolumn{1}{c}{$\Delta U_t$}\\
\hline
lncallin    &     -0.0211         \\
            &    (0.0252)         \\
[1em]
lncallout   &     -0.0165         \\
            &    (0.0319)         \\
[1em]
lnrg        &   0.0000130         \\
            &   (0.00238)         \\
[1em]
churn       &      0.0524         \\
            &     (0.102)         \\
[1em]
ntowers     &     -0.0274         \\
            &    (0.0449)         \\
[1em]
ncallees    &      0.0283         \\
            &    (0.0437)         \\
[1em]
Constant      &     -0.0193         \\
            &    (0.0874)         \\
\hline
\(N\)       &         104         \\
\(R^{2}\)   &       0.038         \\
\hline\hline
\multicolumn{2}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> model_compare_F_no_phones.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Predicting Future Unemployment Rates - Cross Validation Model Coefficients}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}\\
\hline
$ U\_{t-1}$          &       1.161\sym{***}&       1.040\sym{***}&       1.351\sym{***}&       2.140\sym{***}&       1.074\sym{***}&       0.991\sym{***}\\
                    &    (0.0669)         &    (0.0871)         &     (0.329)         &     (0.268)         &    (0.0601)         &    (0.0839)         \\
$ U\_{t-1}^2$        &                     &                     &      -0.852         &      -4.051\sym{***}&                     &                     \\
                    &                     &                     &     (1.421)         &     (0.983)         &                     &                     \\
L.Value             &                     &                     &                     &                     &     0.00220\sym{***}&     0.00194\sym{***}\\
                    &                     &                     &                     &                     &  (0.000213)         &  (0.000174)         \\
\_cons              &     0.00906         &      0.0164\sym{*}  &  -0.0000247         &     -0.0428\sym{**} &     -0.0349\sym{***}&     -0.0256\sym{**} \\
                    &   (0.00730)         &   (0.00776)         &    (0.0165)         &    (0.0150)         &   (0.00668)         &   (0.00801)         \\
\hline
Observations        &          96         &         112         &          96         &         112         &          96         &         112         \\
\(R^{2}\)           &       0.703         &       0.730         &       0.704         &       0.773         &       0.813         &       0.812         \\
Adjusted \(R^{2}\)  &       0.700         &       0.728         &       0.697         &       0.769         &       0.809         &       0.808         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize  Coefficients are reported for models trained on each half of the data.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> model_compare_P_no_phones.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Predicting Future Unemployment Rates - Cross Validation Model Coefficients}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}\\
\hline
$ U\_{t-1}$          &       1.123\sym{***}&       1.061\sym{***}&       1.195\sym{***}&       1.599\sym{***}&       1.072\sym{***}&       1.032\sym{***}\\
                    &    (0.0325)         &    (0.0456)         &     (0.152)         &     (0.139)         &    (0.0316)         &    (0.0441)         \\
$ U\_{t-1}^2$        &                     &                     &      -0.301         &      -2.001\sym{***}&                     &                     \\
                    &                     &                     &     (0.615)         &     (0.562)         &                     &                     \\
L.Value             &                     &                     &                     &                     &     0.00119\sym{***}&     0.00103\sym{***}\\
                    &                     &                     &                     &                     &  (0.000169)         &  (0.000149)         \\
\_cons              &    -0.00180         &     0.00304         &    -0.00541         &     -0.0256\sym{***}&     -0.0244\sym{***}&     -0.0183\sym{***}\\
                    &   (0.00343)         &   (0.00407)         &   (0.00788)         &   (0.00748)         &   (0.00423)         &   (0.00430)         \\
\hline
Observations        &         144         &         168         &         144         &         168         &         144         &         168         \\
\(R^{2}\)           &       0.871         &       0.891         &       0.872         &       0.903         &       0.898         &       0.910         \\
Adjusted \(R^{2}\)  &       0.871         &       0.891         &       0.870         &       0.902         &       0.897         &       0.909         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize  Coefficients are reported for models trained on each half of the data.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table*}


==> model_compare_phones_F.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Predicting Future Unemployment Rates - Cross Validation Model Coefficients}
\label{tab:future_preds_regression}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR2}&\multicolumn{1}{c}{AR2}\\
\hline
$U_{t-1}$          &       1.012\sym{***}&       1.060\sym{***}&       1.369\sym{***}&       1.580\sym{***}&       0.988\sym{***}&       1.029\sym{***}&       0.834\sym{***}&       1.137\sym{**} \\
                    &    (0.0675)         &     (0.108)         &     (0.221)         &     (0.284)         &    (0.0648)         &     (0.115)         &     (0.200)         &     (0.362)         \\
$U_{t-2}$          &                     &                     &                     &                     &                     &                     &       0.202         &      -0.295         \\
                    &                     &                     &                     &                     &                     &                     &     (0.232)         &     (0.344)         \\
$\log(inc)$         &     -0.0819\sym{*}  &     -0.0676\sym{*}  &     -0.0855\sym{*}  &     -0.0492         &     -0.0761\sym{*}  &     -0.0646\sym{*}  &      0.0268         &     -0.0622         \\
                    &    (0.0329)         &    (0.0287)         &    (0.0329)         &    (0.0312)         &    (0.0325)         &    (0.0293)         &    (0.0574)         &    (0.0530)         \\
$\log(out)$         &      0.0536         &      0.0586         &      0.0541         &      0.0613         &      0.0427         &      0.0586         &     0.00374         &       0.115         \\
                    &    (0.0430)         &    (0.0495)         &    (0.0439)         &    (0.0480)         &    (0.0424)         &    (0.0493)         &    (0.0526)         &    (0.0946)         \\
$\log(R_g)$         &    -0.00258         &    -0.00185         &    -0.00312         &    -0.00286         &    -0.00321         &    -0.00203         &     -0.0123         &     0.00310         \\
                    &   (0.00628)         &   (0.00373)         &   (0.00619)         &   (0.00376)         &   (0.00601)         &   (0.00366)         &   (0.00839)         &   (0.00819)         \\
churn               &     -0.0458         &       0.136         &     -0.0461         &      0.0943         &       0.189         &       0.288         &      -0.407         &       0.553         \\
                    &     (0.129)         &    (0.0807)         &     (0.126)         &    (0.0877)         &     (0.157)         &     (0.147)         &     (0.354)         &     (0.395)         \\
contacts            &     -0.0865         &      -0.108         &     -0.0902         &      -0.116         &     -0.0438         &     -0.0793         &    -0.00719         &      -0.132         \\
                    &    (0.0770)         &    (0.0559)         &    (0.0774)         &    (0.0595)         &    (0.0784)         &    (0.0556)         &    (0.0840)         &     (0.125)         \\
towers              &      -0.167\sym{***}&      -0.187\sym{***}&      -0.164\sym{***}&      -0.167\sym{***}&      -0.142\sym{**} &      -0.171\sym{***}&      -0.166\sym{**} &      -0.194\sym{*}  \\
                    &    (0.0447)         &    (0.0479)         &    (0.0437)         &    (0.0461)         &    (0.0446)         &    (0.0488)         &    (0.0602)         &    (0.0766)         \\
$U_{t-1}^2$            &                     &                     &      -1.612         &      -1.937         &                     &                     &                     &                     \\
                    &                     &                     &     (0.990)         &     (1.276)         &                     &                     &                     &                     \\
gdp$_{t-1}$             &                     &                     &                     &                     &     0.00128\sym{*}  &    0.000851         &                     &                     \\
                    &                     &                     &                     &                     &  (0.000594)         &  (0.000637)         &                     &                     \\
\_cons              &       0.372\sym{***}&       0.311\sym{***}&       0.358\sym{***}&       0.286\sym{***}&       0.140         &       0.158         &       0.473\sym{**} &       0.123         \\
                    &    (0.0547)         &    (0.0683)         &    (0.0547)         &    (0.0560)         &     (0.120)         &     (0.132)         &     (0.172)         &     (0.247)         \\
\hline
Observations        &          96         &         112         &          96         &         112         &          96         &         112         &          48         &          56         \\
\(R^{2}\)           &       0.847         &       0.868         &       0.849         &       0.876         &       0.853         &       0.870         &       0.833         &       0.780         \\
Adjusted \(R^{2}\)  &       0.834         &       0.859         &       0.835         &       0.866         &       0.839         &       0.859         &       0.799         &       0.743         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize  Coefficients are reported for models trained on each half of the data.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table*}


==> model_compare_phones_F_pca.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Predicting Future Unemployment Rates - Cross Validation Model Coefficients}
\label{tab:future_preds_regression}
\begin{tabular}{l*{6}{c}}
\hline\hline
& \multicolumn{6}{c}{Model Estimates with out CDR Data} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}\\
\hline
$ U_{t-1}$          &       1.161\sym{***}&       1.040\sym{***}&       1.351\sym{***}&       2.140\sym{***}&       1.074\sym{***}&       0.991\sym{***}\\
                    &    (0.0669)         &    (0.0871)         &     (0.329)         &     (0.268)         &    (0.0601)         &    (0.0839)         \\
$ U_{t-1}^2$        &                     &                     &      -0.852         &      -4.051\sym{***}&                     &                     \\
                    &                     &                     &     (1.421)         &     (0.983)         &                     &                     \\
gdp$_{t-1}$            &                     &                     &                     &                     &     0.00220\sym{***}&     0.00194\sym{***}\\
                    &                     &                     &                     &                     &  (0.000213)         &  (0.000174)         \\
\_cons              &     0.00906         &      0.0164\sym{*}  &  -0.0000247         &     -0.0428\sym{**} &     -0.0349\sym{***}&     -0.0256\sym{**} \\
                    &   (0.00730)         &   (0.00776)         &    (0.0165)         &    (0.0150)         &   (0.00668)         &   (0.00801)         \\
\hline
Observations        &          96         &         112         &          96         &         112         &          96         &         112         \\
\(R^{2}\)           &       0.703         &       0.730         &       0.704         &       0.773         &       0.813         &       0.812         \\
Adjusted \(R^{2}\)  &       0.700         &       0.728         &       0.697         &       0.769         &       0.809         &       0.808         \\
\hline\hline
& \multicolumn{6}{c}{Model Estimates with CDR Data} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}\\
\hline
$ U_{t-1}$          &       1.074\sym{***}&       1.135\sym{***}&       1.490\sym{***}&       1.877\sym{***}&       1.058\sym{***}&       1.070\sym{***}\\
                    &    (0.0608)         &     (0.103)         &     (0.272)         &     (0.300)         &    (0.0583)         &     (0.114)         \\
CDR$_t$                 &     -0.0137\sym{***}&     -0.0117\sym{***}&     -0.0140\sym{***}&     -0.0102\sym{***}&    -0.00716\sym{**} &    -0.00697\sym{*}  \\
                    &   (0.00159)         &   (0.00180)         &   (0.00154)         &   (0.00211)         &   (0.00235)         &   (0.00309)         \\
$ U_{t-1}^2$        &                     &                     &      -1.870         &      -2.775\sym{*}  &                     &                     \\
                    &                     &                     &     (1.229)         &     (1.314)         &                     &                     \\
gdp$_{t-1}$              &                     &                     &                     &                     &     0.00147\sym{***}&     0.00108\sym{**} \\
                    &                     &                     &                     &                     &  (0.000324)         &  (0.000380)         \\
\_cons              &      0.0208\sym{***}&      0.0122         &     0.00110         &     -0.0278         &     -0.0141         &    -0.00932         \\
                    &   (0.00598)         &   (0.00819)         &    (0.0130)         &    (0.0155)         &   (0.00965)         &   (0.00655)         \\
\hline
Observations        &          96         &         112         &          96         &         112         &          96         &         112         \\
\(R^{2}\)           &       0.801         &       0.814         &       0.805         &       0.833         &       0.828         &       0.825         \\
Adjusted \(R^{2}\)  &       0.797         &       0.811         &       0.798         &       0.828         &       0.822         &       0.821         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize  Coefficients are reported for models trained on each half of the data.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table*}


==> model_compare_phones_P.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Predicting Present Unemployment Rates - Cross Validation Model Coefficients}
\label{tab:present_preds_regression}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR2}&\multicolumn{1}{c}{AR2}\\
\hline
$ U_{t-1}$          &       1.040\sym{***}&       1.071\sym{***}&       1.163\sym{***}&       1.272\sym{***}&       1.039\sym{***}&       1.084\sym{***}&       1.168\sym{***}&       1.194\sym{***}\\
                    &    (0.0329)         &    (0.0374)         &     (0.130)         &     (0.129)         &    (0.0330)         &    (0.0367)         &    (0.0956)         &     (0.131)         \\
$ U_{t-2}$          &                     &                     &                     &                     &                     &                     &      -0.110         &      -0.146         \\
                    &                     &                     &                     &                     &                     &                     &     (0.112)         &     (0.158)         \\
$\log(inc)$         &     -0.0532\sym{**} &     -0.0538\sym{**} &     -0.0557\sym{**} &     -0.0493\sym{**} &     -0.0514\sym{*}  &     -0.0562\sym{**} &     -0.0222         &     -0.0564\sym{*}  \\
                    &    (0.0198)         &    (0.0171)         &    (0.0203)         &    (0.0170)         &    (0.0201)         &    (0.0170)         &    (0.0288)         &    (0.0229)         \\
$\log(out)$         &     0.00612         &     -0.0198         &     0.00575         &     -0.0163         &     0.00235         &     -0.0143         &    -0.00869         &      0.0203         \\
                    &    (0.0266)         &    (0.0241)         &    (0.0267)         &    (0.0240)         &    (0.0269)         &    (0.0242)         &    (0.0328)         &    (0.0368)         \\
$\log(r_g)$         &    -0.00162         &    -0.00379         &    -0.00175         &    -0.00390         &    -0.00170         &    -0.00351         &   -0.000807         &    -0.00133         \\
                    &   (0.00368)         &   (0.00207)         &   (0.00367)         &   (0.00212)         &   (0.00368)         &   (0.00207)         &   (0.00466)         &   (0.00331)         \\
churn               &     -0.0905\sym{*}  &     -0.0270         &     -0.0900\sym{*}  &     -0.0226         &     -0.0580         &     -0.0977         &     -0.0925         &      0.0130         \\
                    &    (0.0451)         &    (0.0392)         &    (0.0451)         &    (0.0387)         &    (0.0524)         &    (0.0532)         &    (0.0723)         &    (0.0602)         \\
contacts            &      0.0319         &      0.0276         &      0.0337         &      0.0205         &      0.0424         &     0.00257         &      0.0492         &     -0.0646         \\
                    &    (0.0431)         &    (0.0373)         &    (0.0430)         &    (0.0365)         &    (0.0454)         &    (0.0397)         &    (0.0590)         &    (0.0625)         \\
towers              &      -0.111\sym{***}&     -0.0755\sym{**} &      -0.110\sym{***}&     -0.0691\sym{**} &      -0.100\sym{***}&     -0.0932\sym{***}&      -0.128\sym{**} &      -0.116\sym{**} \\
                    &    (0.0282)         &    (0.0229)         &    (0.0284)         &    (0.0220)         &    (0.0295)         &    (0.0255)         &    (0.0404)         &    (0.0384)         \\
$ U_{t-1}^2$            &                     &                     &      -0.523         &      -0.745         &                     &                     &                     &                     \\
                    &                     &                     &     (0.538)         &     (0.524)         &                     &                     &                     &                     \\
gdp$_{t-1}$             &                     &                     &                     &                     &    0.000300         &   -0.000601         &                     &                     \\
                    &                     &                     &                     &                     &  (0.000313)         &  (0.000327)         &                     &                     \\
\_cons              &       0.172\sym{***}&       0.110\sym{*}  &       0.164\sym{***}&      0.0955\sym{*}  &       0.123         &       0.212\sym{**} &       0.164\sym{**} &       0.228\sym{**} \\
                    &    (0.0408)         &    (0.0441)         &    (0.0410)         &    (0.0436)         &    (0.0634)         &    (0.0719)         &    (0.0539)         &    (0.0741)         \\
\hline
Observations        &         144         &         168         &         144         &         168         &         144         &         168         &          96         &         112         \\
\(R^{2}\)           &       0.912         &       0.933         &       0.913         &       0.935         &       0.913         &       0.934         &       0.926         &       0.930         \\
Adjusted \(R^{2}\)  &       0.908         &       0.930         &       0.908         &       0.931         &       0.908         &       0.931         &       0.919         &       0.925         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize Coefficients are reported for models trained on each half of the data.}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table*}


==> model_compare_phones_P_pca.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Predicting Present Unemployment Rates - Cross Validation Model Coefficients}
\label{tab:present_preds_regression}
\begin{tabular}{l*{6}{c}}
\hline\hline
& \multicolumn{6}{c}{Model Estimates with out CDR Data} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}\\
\hline
$ U_{t-1}$          &       1.123\sym{***}&       1.061\sym{***}&       1.195\sym{***}&       1.599\sym{***}&       1.072\sym{***}&       1.032\sym{***}\\
                    &    (0.0325)         &    (0.0456)         &     (0.152)         &     (0.139)         &    (0.0316)         &    (0.0441)         \\
$ U_{t-1}^2$        &                     &                     &      -0.301         &      -2.001\sym{***}&                     &                     \\
                    &                     &                     &     (0.615)         &     (0.562)         &                     &                     \\
gdp$_{t-1}$              &                     &                     &                     &                     &     0.00119\sym{***}&     0.00103\sym{***}\\
                    &                     &                     &                     &                     &  (0.000169)         &  (0.000149)         \\
\_cons              &    -0.00180         &     0.00304         &    -0.00541         &     -0.0256\sym{***}&     -0.0244\sym{***}&     -0.0183\sym{***}\\
                    &   (0.00343)         &   (0.00407)         &   (0.00788)         &   (0.00748)         &   (0.00423)         &   (0.00430)         \\
\hline
Observations        &         144         &         168         &         144         &         168         &         144         &         168         \\
\(R^{2}\)           &       0.871         &       0.891         &       0.872         &       0.903         &       0.898         &       0.910         \\
Adjusted \(R^{2}\)  &       0.871         &       0.891         &       0.870         &       0.902         &       0.897         &       0.909         \\
\hline\hline
& \multicolumn{6}{c}{Model Estimates with CDR Data} \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 Quad}&\multicolumn{1}{c}{AR1 GDP}&\multicolumn{1}{c}{AR1 GDP}\\
\hline
$ U_{t-1}$          &       1.064\sym{***}&       1.076\sym{***}&       1.180\sym{***}&       1.395\sym{***}&       1.056\sym{***}&       1.062\sym{***}\\
                    &    (0.0330)         &    (0.0389)         &     (0.146)         &     (0.139)         &    (0.0323)         &    (0.0403)         \\
CDR$_t$                 &    -0.00597\sym{***}&    -0.00605\sym{***}&    -0.00602\sym{***}&    -0.00534\sym{***}&    -0.00313\sym{**} &    -0.00481\sym{***}\\
                    &  (0.000928)         &  (0.000842)         &  (0.000925)         &  (0.000917)         &   (0.00120)         &   (0.00120)         \\
$ U_{t-1}^2$        &                     &                     &      -0.486         &      -1.192\sym{*}  &                     &                     \\
                    &                     &                     &     (0.586)         &     (0.566)         &                     &                     \\
gdp$_{t-1}$            &                     &                     &                     &                     &    0.000855\sym{***}&    0.000390         \\
                    &                     &                     &                     &                     &  (0.000225)         &  (0.000211)         \\
\_cons              &     0.00434         &     0.00290         &    -0.00144         &     -0.0141         &     -0.0148\sym{*}  &    -0.00516         \\
                    &   (0.00338)         &   (0.00350)         &   (0.00767)         &   (0.00750)         &   (0.00591)         &   (0.00539)         \\
\hline
Observations        &         144         &         168         &         144         &         168         &         144         &         168         \\
\(R^{2}\)           &       0.893         &       0.918         &       0.894         &       0.922         &       0.902         &       0.920         \\
Adjusted \(R^{2}\)  &       0.892         &       0.917         &       0.891         &       0.920         &       0.900         &       0.918         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize  Coefficients are reported for models trained on each half of the data.}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table*}


==> oos_pred.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption*{Predicting Out of Sample Unemployment Rates}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{$U_t$}&\multicolumn{1}{c}{$\Delta U_t$}\\
\hline
$\hat{U_t}$         &       1.067\sym{***}&                     \\
                    &    (0.0501)         &                     \\
$\Delta\hat{U_t}$  &                     &       1.594\sym{***}\\
                    &                     &     (0.191)         \\
Constant              &      0.0281\sym{***}&      0.0207\sym{***}\\
                    &   (0.00516)         &   (0.00120)         \\
\hline
Observations        &         208         &         208         \\
\(R^{2}\)           &       0.688         &       0.252         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize Predictions relative to a base quarter of Y2008 Q1.}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> pca_loadings.tex <==
\begin{table*}[htbp]\centering 
\caption{PCA Loadings.  Significant elements are bolded.}
\label{tab:PCA_loadings}
 \begin{tabular}{l*{8}{c}} 
\hline\hline
                     &       Comp1 &       Comp2 &       Comp3 &       Comp4 &       Comp5 &       Comp6 &       Comp7\\
\hline
Calls                &    \textbf{0.47} &   -0.117 &    0.098 &    0.013 &   -0.147 &   \textbf{-0.568} &    \textbf{0.643}\\
Inc                  &    \textbf{0.39} &    \textbf{-0.376}&   -0.020 &    0.232 &    \textbf{0.794} &    0.131 &   -0.054\\
Out                  &    \textbf{0.47} &   -0.095 &    0.142 &    0.008 &   -0.268 &   \textbf{-0.346} &   \textbf{-0.746}\\
Contacts             &    \textbf{0.431} &    -0.096   & 0.284 &    0.167 &   \textbf{-0.406} &    \textbf{0.710} &     0.156\\
Churn                &    0.10 &    0.726 &     \textbf{0.605}  &   0.073 &     0.298  &  -0.046 &   -0.002\\
Towers               &    \textbf{0.388} &    0.247 &   \textbf{-0.308} &    \textbf{-0.802}  &    0.125 &    0.179 &    0.015\\
$R_g$                    &    0.252 &    \textbf{0.487} &   \textbf{-0.652} &    \textbf{0.517} &   -0.065 &    0.015 &   -0.006\\
\hline\hline
\end{tabular}
\end{table*}


==> pca_stats.tex <==
\begin{table*}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{PCA results for call variables.}
\label{tab:PCA_stats}
\begin{tabular}{l*{5}{c}}
\hline\hline \\
Component   & Eigenvalue   & Difference   & Proportion   & Cumulative  \\
\hline
Comp1 & 4.10 & 2.93        & 0.59  & 0.59 \\
Comp2 & 1.17 &  0.31       & 0.17  & 0.75 \\
Comp3  &  0.86 &  0.53        & 0.12  & 0.89 \\
Comp4  &  0.34 &  0.04       & 0.05  & 0.93\\
Comp5  &  0.29 &  0.11        & 0.04  & 0.97 \\
Comp6  &  0.19 &  0.15        & 0.03  & 0.99 \\
Comp7 &  0.04      &  .        & 0.01 &   1.00 \\
\hline\hline
\end{tabular}
\end{table*}

==> rmse_calls.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Added Predictive Power of Mobile Phone Data}
\begin{tabular}{l*{7}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
            &\multicolumn{1}{c}{Q2}&\multicolumn{1}{c}{Q3}&\multicolumn{1}{c}{Q4}&\multicolumn{1}{c}{Q5}&\multicolumn{1}{c}{Q6}&\multicolumn{1}{c}{Q7}&\multicolumn{1}{c}{Q8}\\
\hline
unemp\_1     &       0.972\sym{***}&       1.052\sym{***}&       1.052\sym{***}&       1.032\sym{***}&       1.045\sym{***}&       1.084\sym{***}&       1.052\sym{***}\\
            &    (0.0850)         &    (0.0649)         &    (0.0649)         &    (0.0812)         &    (0.0767)         &    (0.0567)         &    (0.0649)         \\
[1em]
lncallin    &     -0.0886\sym{*}  &     -0.0772\sym{*}  &     -0.0772\sym{*}  &     -0.0365         &     -0.0908\sym{**} &     -0.0679         &     -0.0772\sym{*}  \\
            &    (0.0365)         &    (0.0320)         &    (0.0320)         &    (0.0388)         &    (0.0332)         &    (0.0354)         &    (0.0320)         \\
[1em]
lncallout   &     -0.0384         &     -0.0133         &     -0.0133         &     -0.0371         &      0.0387         &      0.0318         &     -0.0133         \\
            &    (0.0527)         &    (0.0473)         &    (0.0473)         &    (0.0589)         &    (0.0548)         &    (0.0477)         &    (0.0473)         \\
[1em]
lnrg        &    -0.00212         &    -0.00219         &    -0.00219         &    -0.00292         &    -0.00439         &   -0.000697         &    -0.00219         \\
            &   (0.00455)         &   (0.00314)         &   (0.00314)         &   (0.00330)         &   (0.00399)         &   (0.00302)         &   (0.00314)         \\
[1em]
churn       &       0.288         &      -0.173\sym{***}&      -0.173\sym{***}&      -0.439\sym{***}&      -0.149\sym{**} &      -0.147\sym{**} &      -0.173\sym{***}\\
            &     (0.193)         &    (0.0510)         &    (0.0510)         &    (0.0955)         &    (0.0557)         &    (0.0522)         &    (0.0510)         \\
[1em]
ncallees    &       0.234\sym{**} &      0.0906         &      0.0906         &       0.108         &      0.0803         &     -0.0534         &      0.0906         \\
            &    (0.0824)         &    (0.0597)         &    (0.0597)         &    (0.0666)         &    (0.0840)         &    (0.0660)         &    (0.0597)         \\
[1em]
ntowers     &      -0.234\sym{***}&      -0.246\sym{***}&      -0.246\sym{***}&      -0.160\sym{**} &      -0.305\sym{***}&      -0.141\sym{***}&      -0.246\sym{***}\\
            &    (0.0452)         &    (0.0386)         &    (0.0386)         &    (0.0488)         &    (0.0490)         &    (0.0413)         &    (0.0386)         \\
[1em]
\_cons      &     -0.0620         &       0.340\sym{***}&       0.340\sym{***}&       0.355\sym{***}&       0.403\sym{***}&       0.341\sym{***}&       0.340\sym{***}\\
            &     (0.180)         &    (0.0739)         &    (0.0739)         &    (0.0921)         &    (0.0993)         &    (0.0619)         &    (0.0739)         \\
\hline
\(N\)       &         156         &         208         &         208         &         156         &         156         &         156         &         208         \\
\(R^{2}\)   &       0.823         &       0.857         &       0.857         &       0.868         &       0.876         &       0.867         &       0.857         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize Each quarter is estimated omitting the month being predicted.}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> rmse_calls_future.tex <==

$U_{t-1}$             &       0.972\sym{***}&       1.052\sym{***}&       1.052\sym{***}&       1.032\sym{***}&       1.045\sym{***}&       1.084\sym{***}&       1.052\sym{***}\\
                    &    (0.0850)         &    (0.0649)         &    (0.0649)         &    (0.0812)         &    (0.0767)         &    (0.0567)         &    (0.0649)         \\
[1em]
lncallin            &     -0.0886\sym{*}  &     -0.0772\sym{*}  &     -0.0772\sym{*}  &     -0.0365         &     -0.0908\sym{**} &     -0.0679         &     -0.0772\sym{*}  \\
                    &    (0.0365)         &    (0.0320)         &    (0.0320)         &    (0.0388)         &    (0.0332)         &    (0.0354)         &    (0.0320)         \\
[1em]
lncallout           &     -0.0384         &     -0.0133         &     -0.0133         &     -0.0371         &      0.0387         &      0.0318         &     -0.0133         \\
                    &    (0.0527)         &    (0.0473)         &    (0.0473)         &    (0.0589)         &    (0.0548)         &    (0.0477)         &    (0.0473)         \\
[1em]
lnrg                &    -0.00212         &    -0.00219         &    -0.00219         &    -0.00292         &    -0.00439         &   -0.000697         &    -0.00219         \\
                    &   (0.00455)         &   (0.00314)         &   (0.00314)         &   (0.00330)         &   (0.00399)         &   (0.00302)         &   (0.00314)         \\
[1em]
churn        &       0.288         &      -0.173\sym{***}&      -0.173\sym{***}&      -0.439\sym{***}&      -0.149\sym{**} &      -0.147\sym{**} &      -0.173\sym{***}\\
                    &     (0.193)         &    (0.0510)         &    (0.0510)         &    (0.0955)         &    (0.0557)         &    (0.0522)         &    (0.0510)         \\
[1em]
ncallees     &       0.234\sym{**} &      0.0906         &      0.0906         &       0.108         &      0.0803         &     -0.0534         &      0.0906         \\
                    &    (0.0824)         &    (0.0597)         &    (0.0597)         &    (0.0666)         &    (0.0840)         &    (0.0660)         &    (0.0597)         \\
[1em]
ntowers      &      -0.234\sym{***}&      -0.246\sym{***}&      -0.246\sym{***}&      -0.160\sym{**} &      -0.305\sym{***}&      -0.141\sym{***}&      -0.246\sym{***}\\
                    &    (0.0452)         &    (0.0386)         &    (0.0386)         &    (0.0488)         &    (0.0490)         &    (0.0413)         &    (0.0386)         \\
[1em]
Constant            &     -0.0620         &       0.340\sym{***}&       0.340\sym{***}&       0.355\sym{***}&       0.403\sym{***}&       0.341\sym{***}&       0.340\sym{***}\\
                    &     (0.180)         &    (0.0739)         &    (0.0739)         &    (0.0921)         &    (0.0993)         &    (0.0619)         &    (0.0739)         \\
\hline
Observations        &         156         &         208         &         208         &         156         &         156         &         156         &         208         \\
\(R^{2}\)           &       0.823         &       0.857         &       0.857         &       0.868         &       0.876         &       0.867         &       0.857         \\
Adjusted \(R^{2}\)  &       0.814         &       0.852         &       0.852         &       0.862         &       0.870         &       0.860         &       0.852         \\


==> rmse_calls_present.tex <==

$U_{t-1}$             &       1.043\sym{***}&       1.022\sym{***}&       1.044\sym{***}&       1.047\sym{***}&       1.027\sym{***}&       1.063\sym{***}&       1.029\sym{***}\\
                    &    (0.0303)         &    (0.0307)         &    (0.0267)         &    (0.0283)         &    (0.0297)         &    (0.0251)         &    (0.0325)         \\
[1em]
lncallin            &     -0.0568\sym{**} &     -0.0627\sym{***}&     -0.0578\sym{**} &     -0.0555\sym{**} &     -0.0694\sym{**} &     -0.0493\sym{**} &     -0.0433\sym{*}  \\
                    &    (0.0206)         &    (0.0186)         &    (0.0178)         &    (0.0182)         &    (0.0210)         &    (0.0189)         &    (0.0208)         \\
[1em]
lncallout           &     -0.0583\sym{*}  &     -0.0157         &     -0.0422         &     -0.0518\sym{*}  &     -0.0243         &     -0.0497\sym{*}  &     -0.0205         \\
                    &    (0.0231)         &    (0.0271)         &    (0.0217)         &    (0.0234)         &    (0.0241)         &    (0.0238)         &    (0.0227)         \\
lnrg                &   -0.000725         &    -0.00233         &    -0.00192         &    -0.00193         &    -0.00201         &    -0.00146         &    -0.00173         \\
                    &   (0.00219)         &   (0.00207)         &   (0.00186)         &   (0.00193)         &   (0.00211)         &   (0.00192)         &   (0.00192)         \\
[1em]
churn        &     -0.0211         &    -0.00967         &     -0.0324         &    -0.00513         &     -0.0458\sym{*}  &     -0.0259         &      -0.134\sym{***}\\
                    &    (0.0215)         &    (0.0223)         &    (0.0199)         &    (0.0236)         &    (0.0212)         &    (0.0243)         &    (0.0266)         \\
[1em]
ncallees     &       0.188\sym{***}&       0.106\sym{**} &       0.142\sym{***}&       0.141\sym{***}&       0.123\sym{**} &       0.142\sym{**} &       0.113\sym{**} \\
                    &    (0.0340)         &    (0.0406)         &    (0.0342)         &    (0.0351)         &    (0.0445)         &    (0.0426)         &    (0.0364)         \\
[1em]
ntowers      &      -0.113\sym{***}&      -0.132\sym{***}&      -0.129\sym{***}&      -0.132\sym{***}&      -0.144\sym{***}&      -0.124\sym{***}&      -0.101\sym{***}\\
                    &    (0.0218)         &    (0.0187)         &    (0.0186)         &    (0.0201)         &    (0.0224)         &    (0.0238)         &    (0.0194)         \\
[1em]
Constant            &     -0.0294         &      0.0788         &      0.0486         &      0.0386         &      0.0967         &      0.0360         &      0.0896\sym{*}  \\
                    &    (0.0502)         &    (0.0468)         &    (0.0411)         &    (0.0427)         &    (0.0517)         &    (0.0414)         &    (0.0441)         \\
\hline
Observations        &         260         &         260         &         312         &         260         &         260         &         260         &         260         \\
\(R^{2}\)           &       0.925         &       0.923         &       0.926         &       0.935         &       0.927         &       0.930         &       0.922         \\
Adjusted \(R^{2}\)  &       0.923         &       0.921         &       0.925         &       0.933         &       0.925         &       0.928         &       0.920         \\


==> rmse_solo_future.tex <==
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{1}{c}{Y1Q2}&\multicolumn{1}{c}{Y1Q3}&\multicolumn{1}{c}{Y1Q4}&\multicolumn{1}{c}{Y1Q1}&\multicolumn{1}{c}{Y1Q2}&\multicolumn{1}{c}{Y1Q3}&\multicolumn{1}{c}{Y1Q4}\\
\hline \\
 \multicolumn{8}{l}{\textbf{Predictions Without Phone Data:}}\\
[1em]
$U_{t-1}$             &       1.031\sym{***}&       1.089\sym{***}&       1.089\sym{***}&       1.082\sym{***}&       1.104\sym{***}&       1.104\sym{***}&       1.089\sym{***}\\
                    &    (0.0737)         &    (0.0631)         &    (0.0631)         &    (0.0763)         &    (0.0734)         &    (0.0595)         &    (0.0631)         \\
[1em]
Constant            &      0.0297\sym{***}&      0.0138\sym{*}  &      0.0138\sym{*}  &      0.0173\sym{*}  &      0.0100         &     0.00213         &      0.0138\sym{*}  \\
                    &   (0.00709)         &   (0.00596)         &   (0.00596)         &   (0.00736)         &   (0.00688)         &   (0.00527)         &   (0.00596)         \\
\hline
Observations        &         156         &         208         &         208         &         156         &         156         &         156         &         208         \\
\(R^{2}\)           &       0.733         &       0.717         &       0.717         &       0.691         &       0.701         &       0.789         &       0.717         \\
Adjusted \(R^{2}\)  &       0.731         &       0.715         &       0.715         &       0.689         &       0.699         &       0.787         &       0.715         \\


==> rmse_solo_present.tex <==
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{1}{c}{Y1Q2}&\multicolumn{1}{c}{Y1Q3}&\multicolumn{1}{c}{Y1Q4}&\multicolumn{1}{c}{Y1Q1}&\multicolumn{1}{c}{Y1Q2}&\multicolumn{1}{c}{Y1Q3}&\multicolumn{1}{c}{Y1Q4}\\
\hline \\
 \multicolumn{8}{l}{\textbf{Predictions Without Phone Data:}}\\
[1em]
$U_{t-1}$             &       1.081\sym{***}&       1.075\sym{***}&       1.087\sym{***}&       1.106\sym{***}&       1.081\sym{***}&       1.113\sym{***}&       1.044\sym{***}\\
                    &    (0.0326)         &    (0.0339)         &    (0.0309)         &    (0.0326)         &    (0.0354)         &    (0.0318)         &    (0.0351)         \\
[1em]
Constant            &     0.00467         &     0.00468         &     0.00118         &   -0.000369         &     0.00260         &    -0.00402         &     0.00178         \\
                    &   (0.00318)         &   (0.00337)         &   (0.00291)         &   (0.00317)         &   (0.00330)         &   (0.00292)         &   (0.00307)         \\
\hline
Observations        &         260         &         260         &         312         &         260         &         260         &         260         &         260         \\
\(R^{2}\)           &       0.887         &       0.877         &       0.882         &       0.886         &       0.874         &       0.895         &       0.880         \\
Adjusted \(R^{2}\)  &       0.887         &       0.876         &       0.882         &       0.885         &       0.873         &       0.895         &       0.880         \\


==> state_unemp_correlations.tex <==
\begin{table*}[htbp]\centering
{\fontsize{7pt}{7pt}\selectfont
\caption{Correlations between mass layoff and unemployment and the state level.}
\label{tab:state_ml_correlations}
\begin{tabular}{l *{5}{p{3cm}}} 
\hline \hline
State & Mass Layoff Events vs. Unemp. Rate & Mass Layoff Events vs. Unemp. Claims & Mass Layoff Claims vs. Unemp. Rate & Mass Layoff Claims vs. Unemp. Claims \\
\hline
Alabama & 0.27 & 0.27 & 0.24 & 0.24 \\ 
Alaska & 0.13 & 0.23 & 0.04 & 0.17 \\ 
Arizona & 0.36 & 0.35 & 0.21 & 0.21 \\ 
Arkansas & 0.37 & 0.38 & 0.25 & 0.27 \\ 
California & 0.44 & 0.42 & 0.30 & 0.27 \\ 
Colorado & 0.40 & 0.39 & 0.35 & 0.33 \\ 
Connecticut & 0.27 & 0.28 & 0.15 & 0.16 \\ 
Delaware & 0.41 & 0.40 & -0.22 & -0.23 \\ 
District of Columbia & -0.38 & -0.36 & -0.46 & -0.50 \\ 
Florida & 0.69 & 0.70 & 0.67 & 0.67 \\ 
Georgia & 0.42 & 0.42 & 0.30 & 0.30 \\ 
Hawaii & 0.46 & 0.46 & 0.37 & 0.36 \\ 
Idaho & 0.31 & 0.31 & 0.32 & 0.28 \\ 
Illinois & 0.48 & 0.49 & 0.50 & 0.51 \\ 
Indiana & 0.33 & 0.34 & 0.19 & 0.20 \\ 
Iowa & 0.23 & 0.24 & 0.18 & 0.19 \\ 
Kansas & 0.33 & 0.34 & 0.25 & 0.25 \\ 
Kentucky & 0.48 & 0.48 & 0.31 & 0.32 \\ 
Louisiana & 0.44 & 0.45 & 0.43 & 0.43 \\ 
Maine & 0.08 & 0.08 & 0.06 & 0.05 \\ 
Maryland & 0.10 & 0.12 & 0.03 & 0.04 \\ 
Massachusetts & 0.12 & 0.12 & 0.09 & 0.09 \\ 
Michigan & 0.16 & 0.16 & 0.09 & 0.09 \\ 
Minnesota & 0.25 & 0.25 & 0.10 & 0.10 \\ 
Mississippi & 0.29 & 0.30 & 0.26 & 0.28 \\ 
Missouri & 0.31 & 0.31 & 0.12 & 0.11 \\ 
Montana & 0.34 & 0.38 & 0.26 & 0.27 \\ 
Nebraska & 0.15 & 0.13 & 0.11 & 0.10 \\ 
Nevada & 0.65 & 0.64 & 0.43 & 0.41 \\ 
New Hampshire & 0.30 & 0.28 & 0.11 & 0.08 \\ 
New Jersey & 0.28 & 0.28 & 0.17 & 0.17 \\ 
New Mexico & 0.25 & 0.32 & 0.08 & 0.16 \\ 
New York & 0.34 & 0.36 & 0.28 & 0.29 \\ 
North Carolina & 0.51 & 0.47 & 0.44 & 0.41 \\ 
North Dakota & 0.30 & 0.31 & 0.10 & 0.12 \\ 
Ohio & 0.25 & 0.25 & 0.15 & 0.15 \\ 
Oklahoma & 0.27 & 0.27 & 0.11 & 0.10 \\ 
Oregon & 0.39 & 0.40 & 0.33 & 0.33 \\ 
Pennsylvania & 0.40 & 0.41 & 0.33 & 0.34 \\ 
Puerto Rico & 0.17 & 0.22 & 0.01 & 0.05 \\ 
Rhode Island & -0.07 & -0.08 & -0.19 & -0.19 \\ 
South Carolina & 0.29 & 0.27 & 0.11 & 0.08 \\ 
South Dakota & 0.60 & 0.58 & 0.15 & 0.12 \\ 
Tennessee & 0.42 & 0.43 & 0.35 & 0.36 \\ 
Texas & 0.51 & 0.45 & 0.39 & 0.32 \\ 
Utah & 0.38 & 0.43 & 0.34 & 0.37 \\ 
Vermont & 0.31 & 0.32 & 0.22 & 0.23 \\ 
Virginia & 0.44 & 0.39 & 0.20 & 0.15 \\ 
Washington & 0.42 & 0.42 & 0.39 & 0.35 \\ 
West Virginia & 0.37 & 0.38 & 0.26 & 0.27 \\ 
Wisconsin & 0.34 & 0.34 & 0.27 & 0.26 \\ 
Wyoming & - & - & - & - \\ 
\hline \hline
\end{tabular}}
\end{table*}

==> tableS1.tex <==
\begin{table*}[t]\centering
%\vspace*{-16cm}
%\begin{sideways}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
{\fontsize{7pt}{7pt}\selectfont
\caption{Regression Results - Social and Mobility Measures.}
\label{tab:micro_regression}
\begin{tabular}{l*{9}{c}}
\hline\hline \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}&\multicolumn{1}{c}{(9)}\\
                    &\multicolumn{1}{c}{Log(calls)}&\multicolumn{1}{c}{Log(inc)}&\multicolumn{1}{c}{Log(out)}&\multicolumn{1}{c}{contacts}&\multicolumn{1}{c}{to town}&\multicolumn{1}{c}{churn}&\multicolumn{1}{c}{Log(towers)}&\multicolumn{1}{c}{Log($R_g$})&\multicolumn{1}{c}{Log($R_1$)}\\
\hline
\\
\multicolumn{10}{l}{\textbf{Panel A: Compared to Random User}} \\
\\
Post-Layoff Dummy &      0.0390\sym{**} &      0.0464\sym{***}&      0.0448\sym{**}       &       0.213\sym{***}& -0.00000264         &      0.0201\sym{***}&      0.0179  &      0.0657\sym{*}  &      0.0588\sym{*} \\
                    &    (0.0155)         &    (0.0170)         &    (0.0193)         &    (0.0124)           &  (0.000135)         &   (0.00592) &    (0.0721)       &      (0.0337)         &    (0.0352)                \\
[1em]
Laidoff Dummy * Post-Layoff Months&      -0.415\sym{***}&      -0.335\sym{***}&      -0.446\sym{***}&      -0.785\sym{*}  &     -0.0478\sym{***}&      0.0368\sym{**} &      -0.171\sym{***}  &       -0.226\sym{**} &      -0.262\sym{**} \\
                     &    (0.0679)         &    (0.0738)         &    (0.0747)       &     (0.458)         &    (0.0136)         &    (0.0167)       &    (0.0550)             &     (0.106)         &     (0.116)              \\\\
\hline \\
Observations        &   10011         &        9742         &        9456           &       10011         &       10011         &       10011     &       10011        &      6922         &        6908            \\
R-Squared           &       0.828         &       0.805         &       0.803           &       0.923         &       0.892         &       0.338          &       0.812           &         0.655         &       0.657          \\\\
\hline \hline
\\
\\
\multicolumn{10}{l}{\textbf{Panel B: Comparison to Non-laidoff Town Users}} \\
\\

Post-Layoff Dummy &       0.0511\sym{***}&      0.0497\sym{***}&      0.0574\sym{***}        &       0.454\sym{***}&   -0.000999         &      0.0301\sym{***}  &     0.00973   &  0.0345\sym{**} &      0.0371\sym{**} \\
                    &    (0.0106)         &    (0.0122)         &    (0.0118)         &     (0.110)         &   (0.00188)         &   (0.00368)      &   (0.00935)          &    (0.0166)         &    (0.0175)             \\
[1em]
Laidoff Dummy * Post-Layoff Months&        -0.517\sym{***}&      -0.416\sym{***}&      -0.545\sym{***}&      -1.311\sym{***}&     -0.0499\sym{***}&      0.0312\sym{*} &      -0.207\sym{***} &       -0.199\sym{*}  &      -0.258\sym{**}  \\
                     &    (0.0679)         &    (0.0738)         &    (0.0747)       &     (0.458)         &    (0.0136)         &    (0.0167)       &    (0.0550)             &    (0.106)         &     (0.116)                  \\\\
\hline \\
Observations        &       17506         &       17342         &       17118         &       17506         &       17506         &       17506     &       17506   &       15474         &       15417             \\
R-Squared          &       0.875         &       0.860         &       0.871         &       0.938         &       0.889         &       0.349       &       0.899        &        0.729         &       0.741         \\\\
\hline \hline
\multicolumn{10}{l}{\footnotesize All specifications include user fixed effects.  Robust standard errors clustered by user.}\\
\multicolumn{10}{l}{\footnotesize *, **, and *** denote significance at the 10\%, 5\% and 1\% levels.}\\
\multicolumn{10}{l}{\footnotesize Note that differences in sample sizes are due to zero values in Log transformations.}\\
\end{tabular}}
%\end{sideways}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\end{document}


